DoRA: Domain-Based Self-Supervised Learning Framework for Low-Resource Real Estate Appraisal

The marketplace system connecting demands and supplies has been explored to develop unbiased decision-making in valuing properties. Real estate appraisal serves as one of the high-cost property valuation tasks for financial institutions since it requires domain experts to appraise the estimation based on the corresponding knowledge and the judgment of the market. Existing automated valuation models reducing the subjectivity of domain experts require a large number of transactions for effective evaluation, which is predominantly limited to not only the labeling efforts of transactions but also the generalizability of new developing and rural areas. To learn representations from unlabeled real estate sets, existing self-supervised learning (SSL) for tabular data neglects various important features, and fails to incorporate domain knowledge. In this paper, we propose DoRA, a Domain-based self-supervised learning framework for low-resource Real estate Appraisal. DoRA is pre-trained with an intra-sample geographic prediction as the pretext task based on the metadata of the real estate for equipping the real estate representations with prior domain knowledge. Furthermore, inter-sample contrastive learning is employed to generalize the representations to be robust for limited transactions of downstream tasks. Our benchmark results on three property types of real-world transactions show that DoRA significantly outperforms the SSL baselines for tabular data, the graph-based methods, and the supervised approaches in the few-shot scenarios by at least 7.6% for MAPE, 11.59% for MAE, and 3.34% for HR10%. We expect DoRA to be useful to other financial practitioners with similar marketplace applications who need general models for properties that are newly built and have limited records. The source code is available at https://github.com/wwweiwei/DoRA.

==> Section/6-Discussion.tex <==
\section{Discussion}
\textit{Significance.}
We have solved a critical domain problem that heavily relies on both domain knowledge and large amounts of annotated in-domain data in property valuations.
The significance of DoRA lies in three aspects.
First, DoRA can benefit all appraisers of real estate by automatically estimating the value of the real estate in areas with limited transactions.
Second, DoRA can be incorporated with domain knowledge.
It combines self-supervised learning and contrastive learning models on tabular data and domain-based pretext tasks to improve model generalizability with unlabeled data.
Third, DoRA is efficient enough for real-time appraisal.
It finishes the real estate appraisal in less than 1 ms, making real-time real estate appraisal practical.

\textit{Limitation.}
The major limitation of this work is the performance with high resource settings.
As shown in Figure \ref{fig:shot}, XGBoost performs slightly better than DoRA in both 50 and 100 shots, which have over 1,000 transactions for each property type.
That is, whether deep learning approaches can outperform tree-based models is still a debatable problem \cite{DBLP:journals/corr/abs-2207-08815,DBLP:journals/inffus/Shwartz-ZivA22}.
We, therefore, focused on low-resource scenarios of real estate appraisal, which is a beneficial task that is hard for supervised models to tackle due to the number of labeled data.
In the future, we plan to extend DoRA to integrate with tree-based approaches to investigate the performance improvement of both low-resource and high-resource scenarios.

\textit{Generalizability.}
DoRA is not limited to real estate appraisal.
It can be easily extended to other property valuation applications, such as rental pricing and security revaluation by designing the pretext task on the unlabeled data.
Moreover, financial institutions can achieve a decent result with limited labeled data and can be deployed to the system due to the efficiency of DoRA, which lowers the cost of extension.

==> Table/10shot.tex <==
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\begin{tabular}{m{25pt}|ccc|ccc|ccc}
    \toprule
    & & \multicolumn{3}{c|}{Building} & \multicolumn{3}{c|}{Apartment} & \multicolumn{3}{c}{House} \\
    \cmidrule{3-11}
    Type & Model & MAPE ($\downarrow$) & HR10\% ($\uparrow$) & HR20\% ($\uparrow$) & MAPE ($\downarrow$) & HR10\% ($\uparrow$) & HR20\% ($\uparrow$) & MAPE ($\downarrow$) & HR10\% ($\uparrow$) & HR20\% ($\uparrow$) \\
    \midrule
    STA & HA  & 44.60$\pm$0.59 & 13.83$\pm$0.25 & 26.76$\pm$0.32 &
                                              43.14$\pm$0.09 & 14.95$\pm$0.22 & 28.57$\pm$0.12 &
                                              45.24$\pm$1.56 & 18.25$\pm$0.25 & \underline{36.40$\pm$0.18}\\
    \midrule
    \multirow{4}{*}{SUP}       & LR         & 58.08$\pm$8.62 & 10.37$\pm$1.91 & 21.06$\pm$3.88 &
                                              60.67$\pm$14.46 & 13.01$\pm$2.13 & 25.13$\pm$4.04 &
                                              76.54$\pm$18.09 & 8.67$\pm$5.92 & 17.19$\pm$10.47\\
                & XGBoost                & \underline{30.65$\pm$3.50} & \textbf{21.91$\pm$1.09} & \textbf{43.02$\pm$2.49} &
                                              28.85$\pm$3.35 & \textbf{23.44$\pm$3.38} & \textbf{45.61$\pm$4.82} &
                                              \textbf{30.70$\pm$0.96} & \textbf{24.85$\pm$0.73} & \textbf{47.69$\pm$2.10}\\
                &\specialcell{DNN} & 38.46$\pm$1.65 & 15.42$\pm$1.93 & 30.66$\pm$3.74 &
                                              38.15$\pm$3.53 & 16.09$\pm$2.12 & 31.33$\pm$3.71 &
                                              33.94$\pm$1.89 & 16.30$\pm$2.32 & 31.87$\pm$3.59\\
                &\specialcell{DNN + CL} & 36.43$\pm$1.01 & 16.75$\pm$1.09 & 31.78$\pm$1.61 &
                                              34.95$\pm$1.57 & 16.18$\pm$1.51 & 32.14$\pm$2.44 &
                                              34.22$\pm$0.32 & 17.05$\pm$2.90 & 33.41$\pm$4.22\\
    \midrule
    \multirow{2}{*}{SSL} & DAE & 44.17$\pm$1.50 & 12.79$\pm$1.89 & 25.71$\pm$2.66 &
                                              41.97$\pm$3.90 & 15.64$\pm$1.10 & 31.31$\pm$2.06 &
                                              39.63$\pm$0.80 & 18.72$\pm$4.48 & 36.61$\pm$9.20\\
                & SubTab     & $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$\\
    \midrule
                & DoRA (Ours)              & \textbf{28.51$\pm$0.90} & \underline{21.84$\pm$1.36} & \underline{41.81$\pm$1.87} &
                                              \textbf{27.95$\pm$0.52} & \underline{21.19$\pm$2.27} & \underline{41.04$\pm$3.59} &
                                              \underline{32.83$\pm$1.42} & \underline{18.75$\pm$0.96} & 36.50$\pm$2.77\\
    \bottomrule
\end{tabular}

==> Table/1shot_2.tex <==
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\begin{tabular}{m{25pt}cc|cc|cc}
    \toprule
    & & \multicolumn{2}{c|}{Building} & \multicolumn{2}{c|}{Apartment} & \multicolumn{2}{c}{House} \\
    \cmidrule{3-8}
    Type & Model & HR20\% ($\uparrow$) & RMSE($\downarrow$) & HR20\% ($\uparrow$) & RMSE ($\downarrow$) & HR20\% ($\uparrow$) & RMSE ($\downarrow$)\\
    \midrule
    STA & HA  & \underline{26.71$\pm$0.24} & 20.24$\pm$0.43 & 26.95$\pm$1.40 &
                                              26.86$\pm$0.84 & 36.40$\pm$0.21 & 12.77$\pm$0.12\\
    \midrule
    \multirow{4}{*}{SUP}& LR                        & 8.86$\pm$8.12 & 38.57$\pm$23.20 & 7.57$\pm$3.47 &
                                              41.95$\pm$6.93 & 8.19$\pm$5.62 & 33.24$\pm$5.01\\
                & XGBoost                & 23.31$\pm$7.75 & 19.52$\pm$4.83 & 33.57$\pm$1.78 &
                                              22.70$\pm$4.49 & 27.54$\pm$6.55 & 15.05$\pm$2.10\\
                &\specialcell{DNN} & 24.21$\pm$3.49 & 20.62$\pm$0.82 & 26.26$\pm$3.78 &
                                              25.08$\pm$2.61 & 30.94$\pm$2.22 & 13.20$\pm$0.56\\
                &\specialcell{DNN + CL} & 23.47$\pm$2.44 & 20.15$\pm$1.08 & 28.80$\pm$5.65 &
                                              23.39$\pm$3.41 & 31.29$\pm$7.36 & 13.00$\pm$0.93 \\
    \midrule
    \multirow{2}{*}{SSL} & DAE & 24.40$\pm$0.40 & 19.86$\pm$2.55 & 28.50$\pm$0.33 &
                                              22.13$\pm$4.46 & \underline{41.20$\pm$1.44} & 11.44$\pm$0.10\\
                & SubTab     & 26.53$\pm$6.17 & \underline{13.96$\pm$4.95} & \underline{34.84$\pm$0.95} &
                                              \textbf{9.10$\pm$0.23} & 28.34$\pm$5.72 & \textbf{9.50$\pm$0.78}\\
    \midrule
                & DoRA (Ours)             & \textbf{28.30$\pm$2.82} & \textbf{11.96$\pm$1.21} & \textbf{37.43$\pm$3.58} & \underline{12.05$\pm$3.06} & \textbf{42.51$\pm$2.84} & \underline{11.25$\pm$0.33}\\
    \bottomrule
\end{tabular}

==> Table/5shot_2.tex <==
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\begin{tabular}{m{25pt}cc|cc|cc}
    \toprule
    & & \multicolumn{2}{c|}{Building} & \multicolumn{2}{c|}{Apartment} & \multicolumn{2}{c}{House} \\
    \cmidrule{3-8}
    Type & Model & HR20\% ($\uparrow$) & RMSE($\downarrow$) & HR20\% ($\uparrow$) & RMSE ($\downarrow$) & HR20\% ($\uparrow$) & RMSE ($\downarrow$)\\
    \midrule
    STA & HA  & 26.75$\pm$0.24 & 20.44$\pm$0.43 & 26.95$\pm$1.40 &
                                              27.63$\pm$0.34 & 36.21$\pm$0.64 & 12.69$\pm$0.09\\
    \midrule
    \multirow{4}{*}{SUP}& LR                        & 19.76$\pm$5.50 & 26.97$\pm$3.74 & 16.95$\pm$7.94 &
                                              37.81$\pm$15.88 & 13.20$\pm$11.89 & 44.20$\pm$36.09\\
                & XGBoost                & 36.26$\pm$6.21 & 13.42$\pm$0.96 & 39.16$\pm$7.92 &
                                              17.49$\pm$3.26 & \textbf{44.08$\pm$3.26} & 14.17$\pm$4.82\\
                &\specialcell{DNN} & 29.27$\pm$3.10 & 17.69$\pm$1.81 & 30.12$\pm$1.47 &
                                              23.98$\pm$2.42 & 33.99$\pm$7.45 & 12.39$\pm$0.79\\
                &\specialcell{DNN + CL} & 28.89$\pm$5.15 & 17.60$\pm$1.79 & 32.17$\pm$2.77 &
                                              21.83$\pm$1.16 & 31.38$\pm$6.51 & 12.84$\pm$0.64 \\
    \midrule
    \multirow{2}{*}{SSL} & DAE & 27.29$\pm$2.71 & 18.22$\pm$2.40 & 30.37$\pm$1.60 &
                                              19.98$\pm$1.56 & 39.09$\pm$7.31 & 11.90$\pm$1.33\\
                & SubTab     & \textbf{42.00$\pm$0.42} & \textbf{9.66$\pm$0.11} & \textbf{43.84$\pm$2.39} &
                                              \textbf{8.32$\pm$0.34} & 42.46$\pm$1.67 & \textbf{6.80$\pm$0.21}\\
    \midrule
                & DoRA (Ours)              & \underline{38.13$\pm$0.83} & \underline{12.34$\pm$0.63} & \underline{39.41$\pm$1.21} &
                                              \underline{15.53$\pm$0.49} & \underline{42.79$\pm$0.20} & \underline{11.27$\pm$0.08}\\
    \bottomrule
\end{tabular}

==> Table/ablation_2.tex <==
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\begin{tabular}{ccccc|cc}
    \toprule
    \specialcell{Pre-Trained\\Datasets} & \specialcell{Pretext\\Task} & CL ($\alpha$) & $d_Z$ & \specialcell{Fine-Tune\\Encoder} & MAE ($\downarrow$) & HR10\% ($\uparrow$) \\
    \midrule
    \midrule
    Building & Town & + (0.7) & 256 & \cmark & 12.05 & 15.25 \\
    \midrule
    All & Town & + (0.7)  & 512 & \cmark & 9.22 & 19.24 \\
    \midrule
    All & Town & + (0.7) & 256 & \xmark & 15.16 & 7.41 \\
    \midrule
    All & Town & - & 256 & \cmark & 11.51 & 13.48 \\
    \midrule
    All & Town & + (0.5) & 256 & \cmark & 12.79 & 14.99 \\
    \midrule
    \midrule
    All & City & + (0.7) & 256 & \cmark & 10.88 & 17.8 \\
    \midrule
    All & Parking Spot & + (0.7) & 256 & \cmark & 11.61 & 14.63 \\
    \midrule
    All & House Age & + (0.7) & 256 & \cmark & 9.64 & 18.43 \\
    \midrule
    All & Floor & + (0.7) & 256 & \cmark & 9.64 & 18.05 \\
    \midrule
    \midrule
    All & Town & + (0.7) & 256 & \cmark & \textbf{7.79} & \textbf{20.16} \\
    \bottomrule
\end{tabular}

% \begin{tabular}{ccccc|ccc}
%     \toprule
%     \specialcell{Pre-Trained\\Datasets} & \specialcell{Pretext\\Task} & CL ($\alpha$) & $d_Z$ & \specialcell{Fine-Tune\\Encoder} & MAPE ($\downarrow$) & MAE ($\downarrow$) & HR10\% ($\uparrow$) \\
%     \midrule
%     \midrule
%     Building & Town & + (0.7) & 256 & \cmark & 37.09 & 12.05 & 15.25 \\
%     \midrule
%     All & Town & + (0.7)  & 512 & \cmark & 33.65 & 9.22 & 19.24 \\
%     \midrule
%     All & Town & + (0.7) & 256 & \xmark & 58.65 & 15.16 & 7.41 \\
%     \midrule
%     All & Town & - & 256 & \cmark & 37.83 & 11.51 & 13.48 \\
%     \midrule
%     All & Town & + (0.5) & 256 & \cmark & 36.37 & 12.79 & 14.99 \\
%     \midrule
%     \midrule
%     All & City & + (0.7) & 256 & \cmark & 36.38 & 10.88 & 17.8 \\
%     \midrule
%     All & Parking Spot & + (0.7) & 256 & \cmark & 38.13 & 11.61 & 14.63 \\
%     \midrule
%     All & House Age & + (0.7) & 256 & \cmark & 32.37 & 9.64 & 18.43 \\
%     \midrule
%     All & Floor & + (0.7) & 256 & \cmark & 34.9 & 9.64 & 18.05 \\
%     \midrule
%     \midrule
%     All & Town & + (0.7) & 256 & \cmark & \textbf{31.85} & \textbf{7.79} & \textbf{20.16} \\
%     \bottomrule
% \end{tabular}

==> Table/data_details.tex <==
\begin{tabular}{c|cc}
    \toprule
    Feature & Feature Type (\#class) & Example \\
    \midrule
    City Name & Category (21) & Taipei city\\
    Town Name & Category (350) & Ren'ai township \\
    Parking spot & Category (2) & True/False (If the house includes a parking spot.) \\
    Studio & Binary & True/False (If the area of the estate is smaller than 8 square meters.) \\
    Details building type & Category (5) & Residential building (11 floors and above), Mansion (10 floors and below) \\
    Main Purpose & Category (1622) & Electromechanical equipment space \\
    Building materials & Category (220) & Rebar, Wood \\
    Management organization & Binary & True/False \\
    Type of parking space & Category (3) & Flat parking spot, Automated parking spot \\
    Elevator & Binary & True/False \\
    First-floor index & Binary &  True/False (If the house is located on the first floor.)\\
    Shop index & Binary &  True/False (If the house is for shop use.)\\
    Housing type & Category (3) & Building, Apartment, House \\
     % col2\_ind & Category(2) &  \\
    Village name & Category (4650) & Zhongshan village \\
    Land use & Category (19) & Residential zone, Forestry land, Mining land \\
    Land Use Designation & Category (16) & Type A building land, Class B building site \\
    Land transfer area & Numerical & 30 \\
    Building transfer area & Numerical & 50 \\
    Number of bedrooms & Numerical & 2 \\
    Number of living rooms & Numerical & 1 \\
    Number of bathroom & Numerical & 3 \\
    Number of total rooms & Numerical & 5 \\
    Parking area & Numerical & 5 \\
    Main building area & Numerical & 100 \\
    Ancillary building area & Numerical  & 10 \\
    Balcony area & Numerical & 5 \\
    House age & Numerical & 10 years \\
    Number of land transaction & Numerical & 1 \\
    Number of building transaction & Numerical &  1 \\
    Number of parking space transactions & Numerical & 2 \\
    Building area without parking area & Numerical & 45 \\
    Single floor area & Numerical & 20 \\
    Floor area ratio (FAR) & Numerical & 10 (Derived by dividing the total area of the building by the total area of the parcel.) \\
    Estate floor & Numerical & 5 \\
    Total floor & Numerical & 10 \\
    Latitude & Numerical & Horizontal lines that measure distance north or south of the equator \\
    Longitude & Numerical & Vertical lines that measure east or west of the meridian in Greenwich, England. \\
    Building coverage ratio & Numerical & 9 \\
    Park count flat & Numerical &  0 \\
    \bottomrule
\end{tabular}

==> Table/data_details_2.tex <==
\begin{tabular}{c|cc}
    \toprule
   Feature & Feature Type (\#class) & Example \\
    \midrule
    YIMBY\_10 & Numerical & 2\\
    YIMBY\_50 & Numerical & 3\\
    YIMBY\_100 & Numerical & 3\\
    YIMBY\_250 & Numerical & 6\\
    YIMBY\_500 & Numerical & 7\\
    YIMBY\_1000 & Numerical & 13\\
    YIMBY\_5000 & Numerical & 28\\
    YIMBY\_10000 & Numerical & 52\\
    \midrule
    NIMBY\_10 & Numerical &  0\\
    NIMBY\_50 & Numerical &  0\\
    NIMBY\_100 & Numerical &  0\\
    NIMBY\_250 & Numerical &  1\\
    NIMBY\_500 & Numerical &  1\\
    NIMBY\_1000 & Numerical &  2\\
    NIMBY\_5000 & Numerical &  3\\
    NIMBY\_10000 & Numerical &  6\\
    \bottomrule
\end{tabular}

==> Table/data_details_3.tex <==
\begin{tabular}{c|cc}
    \toprule
    Feature & Feature Type (\#class) & Example \\
    \midrule
    Land area per town & Numerical & 23.13 (km\textsuperscript{2}) \\
    Population density per town & Numerical & 23835 (\#people/km\textsuperscript{2}) \\
    House price index per quarter & Numerical & 110 \\
    Unemployment rate per quarter & Numerical & 5\% \\
    Economic growth rate per quarter & Numerical & 3\% \\
    Lending rate per quarter & Numerical & 1.9\% \\
    Land transaction count per quarter & Numerical & 163796 \\
    Average land price index per quarter & Numerical & 101 \\
    Steel price index per quarter & Numerical & 1071 \\
    \bottomrule
\end{tabular}

==> Table/datasets_stat.tex <==
\begin{tabular}{c|ccc}
    \toprule
    Sets/Property Type & Building & Apartment & House \\
    \midrule
    \#unlabeled set & 68,283 & 230,410 & 135,820 \\
    \#labeled set & 68,282 & 230,409 & 135,820 \\
    % \#training set & 136,565 & 460,819 & 271,640 \\
    \midrule
    \#validation set & 7,318 & 20,365 & 12,441 \\
    \midrule
    \#testing set & 4,709 & 11,892 & 7,541 \\
    \midrule
    \midrule
    \#total & 148,592 & 493,076 & 291,622 \\
    \bottomrule
\end{tabular}

==> Table/different_pretext_performance.tex <==
\begin{tabular}{c|cccc}
    \toprule
     & Precision ($\uparrow$) & Recall ($\uparrow$) & Macro-F1 ($\uparrow$) & Micro-F1 ($\uparrow$)\\
    \midrule
    Town (Ours) & 0.8721 & 0.8535 & 0.8501 & 0.9584 \\
    City & 0.9303 & 0.9426 & 0.9351 & 0.9930 \\
    \bottomrule
\end{tabular}

==> Table/different_pretext_task.tex <==
\newcommand{\specialcell}[2][c]{
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\begin{tabular}{m{25pt}|ccc|ccc|ccc}
    \toprule
    & & \multicolumn{3}{c|}{Building} & \multicolumn{3}{c|}{Apartment} & \multicolumn{3}{c}{House}\\
    \cmidrule{3-11}
    Pretext Target & Type & MAPE ($\downarrow$) & MAE ($\downarrow$) & HR10\% ($\uparrow$) & MAPE ($\downarrow$) & MAE ($\downarrow$) & HR10\% ($\uparrow$) & MAPE ($\downarrow$) & MAE ($\downarrow$) & HR10\% ($\uparrow$) \\
    \midrule
    Town (Ours) & \multirow{3}{*}{Classification}  & \textbf{38.77} & \textbf{11.16} & \textbf{14.53} & \textbf{33.73} & \textbf{10.51} & \textbf{19.55} & \textbf{33.59} & \textbf{6.53} & \textbf{22.41} \\
    City & & \underline{42.5} & 13.91 & 12.23 & \underline{38.93} & \underline{13.47} & \underline{16.03} & 35.49 & 7.31 & 17.16\\
    Parking Spot & & 46.33 & 15.20 & 12.51 & 40.69 & 31.15 & 14.67 & 37.53 & 10.01 & 19.44 \\
    \midrule
    House Age & \multirow{2}{*}{Regression}  & 44.85 & 13.30 & 13.21 & 40.75 & 17.56 & 14.85 & \underline{34.02} & \underline{7.14} & \underline{19.45} \\
    Floor & & 44.11 & \underline{12.98} & 12.59 & 42.86 & 16.50 & 15.29 & 39.47 & 7.71 & 15.90 \\
    \midrule
    \specialcell[c]{Town + \\House Age} & \specialcell[c]{Classification +\\Regression} & 43.71 & 25.57 & \underline{13.97} & 42.81 & 16.50 & 15.43 & 39.45 & 15.65 & 7.72 \\
    \bottomrule
\end{tabular}

==> Table/feature_ablation.tex <==
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\begin{tabular}{c|ccccc}
    \toprule
    Feature & MAPE ($\downarrow$) & MAE ($\downarrow$) & HR10\% ($\uparrow$)\\
    \midrule
    RF & 44.11 & 13.26 & 12.59 \\ 
    \midrule
    RF + PoI & 33.37 & 16.05 & 18.01 \\
    \midrule
    RF + Econ\&Geo & 41.37 & 12.26 & 13.34 \\
    \midrule
    \midrule
    All & \textbf{31.85} & \textbf{7.79} & \textbf{20.16} \\
    \bottomrule
\end{tabular}

==> Table/few_shot_stat.tex <==
\begin{tabular}{c|ccccc}
    \toprule
    \#shots & 1 & 5 & 10 & 50 & 100 \\
    \midrule
    Building & 22 & 110 & 218 & 1058 & 2108 \\
    \midrule
    Apartment & 19 & 95 & 190 & 950 & 1900 \\
    \midrule
    House & 22 & 106 & 211 & 1051 & 2101 \\
    \bottomrule
\end{tabular}

==> Table/pretext_task_performance.tex <==
\begin{tabular}{c|cccc}
    \toprule
     & Precision ($\uparrow$) & Recall ($\uparrow$) & Macro-F1 ($\uparrow$) & Micro-F1 ($\uparrow$)\\
    \midrule
    DoRA (Ours) & 0.8721 & 0.8535 & 0.8501 & 0.9584 \\
    \bottomrule
\end{tabular}

==> Table/shot_template.tex <==
%%%%% NO USED
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\begin{tabular}{m{25pt}ccc|ccc|ccc}
    \toprule
    & & \multicolumn{3}{c|}{Building} & \multicolumn{3}{c|}{Apartment} & \multicolumn{3}{c}{House} \\
    \cmidrule{3-11}
    Type & Model & \specialcell{MAPE} & \specialcell{Hit10} & \specialcell{Hit20} & \specialcell{MAPE} & \specialcell{Hit10} & \specialcell{Hit20} & \specialcell{MAPE} & \specialcell{Hit10} & \specialcell{Hit20}\\
    \midrule
    \textbf{Sup} & HA  & $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$\\
                & LR                        & $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$\\
                & XGBoost                & $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$\\
                &\specialcell{DNN\\(w/o CL)} & $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$\\
                &\specialcell{DNN\\(w/ CL)} & $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$\\
    \midrule
    \textbf{SSL} & DAE & $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$\\
                & SubTab     & $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$\\
    \midrule
                & DoRA (Ours)              & $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$ &
                                              $\pm$ & $\pm$ & $\pm$\\
    \bottomrule
\end{tabular}
